Generalizations of analogs of theorems of Maizel and Pliss and their application in Shadowing Theory

We generalize two classical results of Maizel and Pliss that describe relations between hyperbolicity properties of linear system of difference equations and its ability to have a bounded solution for every bounded inhomogeneity. We also apply one of this generalizations in shadowing theory of diffeomorphisms to prove that some sort of limit shadowing is equivalent to structural stability.

==> discreteReview.tex <==
\section{Review of existing results}

\newcommand{\Xdiscr}{X}
\newcommand{\Xcont}{\hat{X}}
\newcommand{\Adiscr}{A}
\newcommand{\Acont}{\hat{A}}
\newcommand{\Mdiscr}{M}
\newcommand{\Mcont}{\hat{M}}
\newcommand{\Ldiscr}{L}
\newcommand{\Lcont}{ {\hat{L}} }
\newcommand{\Idiscr}{I}
\newcommand{\Icont}{ {\hat{I}} }
\newcommand{\Lpdiscr}[1]{l_{#1}}
\newcommand{\Lpcont}[1]{L_{#1}}

%Свойство Перрона изучалось многими авторами. Часто его называют свойством допустимости (admissibility).

There are lots of papers devoted to the study of connection between Perron property (which is often called admissibility) and hyperbolicity (which is has form of dichotomy in this sort of papers).

%The first books people usually cite are monograph of Coppel on dichotomies \cite{COPPEL__DICH_IN_STAB_TH} and book of Massera and Sch\"{a}ffer \cite{MASS__LIN_DIF_EQ_AND_FUNC_SPACES}.

The papers mentioned generalize Maizel and/or Pliss theorems in different ways. There are two types of such generalizations -- ones that widen the class of spaces to which theorem can be applied and ones that replaces the Perron property by some similar notion.

We give a here short survey of existing results. We don't want to fall deep into details so some statements of the theorems in this section are not very accurate -- see provided references for exact statements.

%Invertibility of the operator, corresponding to the system of linear difference or differential equations in finite or infinite-dimensional case (see
%\cite{DALKREINSTAB, BASK__INV_FREDHOLM_PROPS_DIF_OPER,
%GOHBERG__DICH_AND_INV,
%GOHBERG__INV_AND_DICH_HALFLINE}).
%
%
%Fredholm properties of the operator, corresponding to the system of linear difference or differential equations in finite or infinite-dimensional case (see \cite{SACKER__SPLITTING, PAL__EXP_DICH_AND_TVS, PAL__EXP_DICH_AND_FRED_OPER, BASK__INV_FREDHOLM_PROPS_DIF_OPER, LAT__DICH_FRED_PROPS_EVOL_EQ, LAT__DICH_TH_EVOL_BIFAM, GOHBERG__DICH_AND_INV,
%GOHBERG__INV_AND_DICH_HALFLINE}).

%There exist concept of "measure chains" that generalizes concepts of difference and differential equations (see \cite{CHRIST__PERSIST_IMPERF_NONAUT_BIF_PATTERNS} )
%Christian P\"{o}tzsche

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

At first we need some definitions. For Banach spaces $A,B$ denote the space of linear operators from $A$ to $B$ by $\Lc(A,B).$ For a Banach space $X$ and set $I$ denote the space of functions from $I$ to $X$ by $X^I.$

Let $\Idiscr$ be either $\Zplus = \setdef{k\in\Zb}{k\geq 0}$ or $\Zminus = \setdef{k\in\Zb}{k\leq 0}$ or $\Zb.$ Let $\Xdiscr$ be a Banach space. Let $\{\Adiscr_k\}_{k\in \Idiscr}$ be a sequence of operators from $\Lc(\Xdiscr,\Xdiscr),$ indexed by integers from $I.$ Consider homogeneous and inhomogeneous equations associated with this sequence.
\begin{IEEEeqnarray}{rCll}
x_{k+1}&=&A_k x_k,\qquad &k\in I, \label{eqs:homdiscr} \\
x_{k+1}&=&A_k x_k + f_{k+1},\qquad &k\in I. \label{eqs:inhomdiscr}
\end{IEEEeqnarray}
Let $\Mdiscr$ be a subspace of $\Xdiscr^\Idiscr.$ Then there is an operator $\Ldiscr\in \Lc(\Mdiscr,\Xdiscr^\Idiscr),$ associated to this system
\begin{equation*} \label{def:discroper}
(\Ldiscr x)_k = x_{k+1} - \Adiscr_kx_k.
\end{equation*}

The similar setup can be made for continuous case. Let $\Icont$ be either $\Rplus = \setdef{k\in\Rb}{k\geq 0}$ or $\Rminus = \setdef{k\in\Rb}{k\leq 0}$ or $\Rb.$ Let $\Xcont$ be Banach space. Let $\Acont:\Icont\to \Lc(\Xcont,\Xcont)$ be an operator-valued function. Consider homogeneous and inhomogeneous equations associated with this function.
\begin{IEEEeqnarray}{rCll}
\dot{x} & = & A(t)x,& t\in \hat{I}, \label{eqs:homcont} \\
\dot{x} & = & A(t)x + f(t),\quad & t\in \hat{I}. \label{eqs:inhomcont}
\end{IEEEeqnarray}
Let $\Mcont$ be a subspace of $\Xcont^{\Icont}.$ Then there is an operator $\Lcont\in \Lc(\Mcont,\Xcont^{\Icont}),$ associated to this system
\begin{equation*} \label{def:contoper}
(\Lcont x)(t) = \dot{x}(t) - \Acont(t)x(t).
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%

Let $\Phi(s,t)$ be the fundamental matrix of the system \eqref{eqs:homcont} and $S(t) = \Phi(t,0)$.

\begin{deffnon}
The system \eqref{eqs:homcont} is said to have an exponential dichotomy on $\hat{I}$ if there is a projection $P$ and constants $K>0,\ \alpha>0$ such that
\begin{IEEEeqnarray}{rcll}
\normop{S(t)PS^{-1}(s)} &\leq& Ke^{-\alpha(t-s)},\quad & s\leq t,\\
\normop{S(t)(I-P)S^{-1}(s)} &\leq& Ke^{-\alpha(s-t)}, & s\geq t.
\end{IEEEeqnarray}
\end{deffnon}
The spaces $P S$ and $(I-P)S$ are called stable and unstable. The definition of exponential dichotomy for system \eqref{eqs:homdiscr} is absolutely analogous. We will denote the fundamental matrices of system \eqref{eqs:homdiscr} by the same letters $\Phi, S$ as in the continuous case.

For Banach spaces $A,B$ denote the space of continuous from $A$ to $B$ by $C(A,B).$
Denote
$$C_b(A,B)=\Lpcont{\infty} \cap C(A,B),$$
$$C_0(A,B)=\setdef{f\in C(A,B) }{ \lim_{t\to\infty} \vmod{f(t)} = 0 }, $$
$$C_{b,0}(A,B)=C(A,B) \cup C_0 (A,B).$$
Let $I$ be an interval in $\Rb$ and $B$ be a Banach space. Denote
$$\Lpcont{p}(I,B) = \setdef{f:A \to B}{ \enbrace{ \int_I \normban{f}_B^p  }^{\frac{1}{p}} },\ p\in [1,\infty),$$
$$\Lpcont{\infty}(I,B) = \setdef{f:A \to B}{ \esssup\limits_{x\in I} \normban{f(x)}_B < \infty }.$$
All these spaces have their analogs in discrete case.

%$\Lpdiscr{p}$ or $\Lpdiscr{\infty}$ or $c_0.$

%%%%%%%%%%%%%%%%%%%%%

\begin{deffnon}
We say that the pair $(U,V)$ of subspaces of $\Xcont^{\Icont}$ is admissible for the system \eqref{eqs:homcont} if for every inhomogeneity from $V$ there exist a solution of the system that belongs to $U.$ This is equivalent to saying (in some situations) that the operator $\Lcont$ is surjective. The similar definition can be made in discrete case.
\end{deffnon}

%%%%%%%%%%%%%%%%%%%%

%link
%We say that the pair $(U,V)$ of subspaces of $\Xcont^\Icont$ is completely admissible (see \cite{SASU__TRANS_INV_SPACES_ASYMPT_PROPS_VAR_EQ_11}) for the system \eqref{eqs:homcont} if for every inhomogeneity $f$ from $V$ there exist only one solution $y$ of the system that belongs to $U.$ This is equivalent to saying (in some situations) that the operator $\Lcont$ is continuously invertible.

%%%%%%%%%%%%%%%%%%%%%

The study of solvability of system \eqref{eqs:inhomdiscr} and \eqref{eqs:inhomcont} can be divided in two parts: when $\Xcont$ (or $\Xdiscr$) is finite dimensional and when it is infinite dimensional. Finite dimensional results usually used in qualitative study of differential equations. %To prove different sorts of stability or existence of homoclinic orbits.
Infinite dimensional results used for the study of PDEs. In case of infinite dimensions the case where operators $A(t)$ or $A_k$ are not uniformly bounded is of special interest.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Finite dimensional case}

%Let $X$ be $\mathbb{C}^n$ or $\Rb^n.$

%%%%%%%%%%%%%%%%%%%%% Perron

%?
The pioneering work establishing connections between dichotomy and admissibility \eqref{eqs:homcont}) is attributed to Perron. In modern terminology, his paper \cite{PERRON} relates the asymptotic properties of solutions of homogeneous equations (in a finite-dimensional space $\Xcont$) to certain properties of operator $\Lcont$ on $C_b(\Rplus,\Xcont).$

\subsubsection{A. Maizel and W. Coppel} %Andrey
%%%%%%%%%%%%%%%%%%%%% Coppel and Maizel

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rplus.$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{MAIZEL} Maizel shows that the pair $( C(\Rplus,\Xcont), C(\Rplus,\Xcont) )$ is admissible for system \eqref{eqs:inhomcont} if and only if it has exponential dichotomy on $\Rplus$.

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb$ and $\Mcont = C_b(\Rb,\Xcont).$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{MAIZEL} Maizel also shows that the operator $\Lcont$ has %continuous
inverse if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rb.$

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb.$
In \cite{COPDFA} Coppel proves that system \eqref{eqs:homcont} has exponential dichotomy on $\Rb$ if and only if it has exponential dichotomy on both $\Rplus$ and $\Rminus$ with projectors $P^+$ and $P^-$ and $P^+ \Xcont \oplus P^- \Xcont = \Xcont.$

\subsubsection{V. Pliss} %Viktor
%%%%%%%%%%%%%%%%%%%%%% Pliss

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb.$
In \cite{PLISSBSILSDE} Pliss shows that the pair $ (C(\Rb,\Xcont),C(\Rb,\Xcont))$ is admissible for system \eqref{eqs:inhomcont} if and only if system \eqref{eqs:homcont} has exponential dichotomy on both $\Rplus$ and $\Rplus$ with projectors $P^+$ and $P^-$ and $P^+ \Xcont + P^- \Xcont = \Xcont.$

\subsubsection{R. Sacker}
%%%%%%%%%%%%%%%%% Sacker abstract

%, Theorem 3,
Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb$ and let $\Mcont$ contain bounded or locally integrable functions.
Let the sequence of operators $\Acont(t)$ be bounded or local integrable.
In \cite{SACKER__SPLITTING} Sacker gives conditions on the system \eqref{eqs:homcont} for time near plus and minus infinity which guarantee that the operator $\Lcont$ is Fredholm. The conditions are closely related to dichotomy properties of the system.

\subsubsection{Kenneth Palmer}
%%%%%%%%%%%%%%%%%%%%%%% Palmer

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb$ and $\Mcont = C^1(\Rb,\Rb^d).$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{PAL__EXP_DICH_AND_TVS} Palmer shows that if the operator $\Lcont$ has exponential dichotomy on both $\Rplus$ and $\Rminus$ than it is Fredholm.

%This result can also be obtained as a consequence of a more general theory due to Sacker \cite{SACKER__SPLITTING}, where the Fredholm index of an operator like L can be computed in terms of the so-called "splitting index" of the matrix $A(t)$.

%In \cite{PAL__EXP_DICH_AND_FRED_OPER} Palmer shows that if $\Acont(t)$ is bounded and continuous and the range of operator \eqref{def:contoper} is closed then when $\Icont$ is a half-line, system \eqref{eqs:homcont} has an exponential dichotomy on $\Icont$ and when $\Icont = \Rb,$ \eqref{eqs:homcont} has exponential dichotomies on both $\Rplus$ and $\Rminus.$ Here $\Mcont$ is a subspace of $C^1(\Rb,\Rb^d)$ of functions that are bounded with their derivatives.
% it must be, in
%fact, Fredholm and even surjective in the half-line case

\subsubsection{A. Ben-Artzi} %Asher
%%%%%%%%%%%%%%%%%%%%% Gohberg
% in "Dichotomy of systems and invertibility of linear ordinary differential operators"
% http://www.google.ru/books?hl=ru&lr=&id=JDC1Qxcwb7YC&oi=fnd&pg=PR7&dq=%22Dichotomy+of+systems+and+invertibility+of+linear+ordinary+differential+operators%22&ots=f5_7ME-uex&sig=pxYNkXJBQgBwSW1LrTcpYM0B-jw&redir_esc=y#v=onepage&q=%22Dichotomy%20of%20systems%20and%20invertibility%20of%20linear%20ordinary%20differential%20operators%22&f=false

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb$ and $\Mcont = \Lpcont{p}(\Rb,\Xcont),$ where $1<p<\infty.$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{GOHBERG__DICH_AND_INV} Ben-Artzi and Gohberg show that the operator $\Lcont$ is invertible if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rb.$

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rb$ and $\Mcont = \Lpcont{p}(\Rb,\Xcont),\ 1<p<\infty.$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{GOHBERG__DICH_AND_INV} Ben-Artzi and Gohberg also show that the operator $\Lcont$ is Fredholm if and only if system \eqref{eqs:homcont} and the system
$$
\dot{x}=-\Acont(-t)x(t),\quad x\in\Rplus
$$
both have exponential dichotomy on $\Rplus.$

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rplus$ and $\Mcont = \Lpcont{p}(\Rplus,\Xcont),$ where $1<p<\infty.$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{GOHBERG__DICH_AND_INV} Ben-Artzi and Gohberg show that the operator $\Lcont$ is Fredholm if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rplus.$

%In that case the operator is proved to be a direct sum of two generators of $C_0$ semigroups, one of which has support on the negative half line and the other on the positive half line.

Consider the case where $\Xcont$ is finite-dimensional, $\Icont = \Rplus$ and $\Mcont = \Lpcont{p}(\Rplus,\Xcont),$ where $1\leq p <\infty.$
Let the sequence of operators $\Acont(t)$ be bounded.
In \cite{GOHBERG__INV_AND_DICH_HALFLINE} Ben-Artzi, Gohberg and Kaashoek show that the operator $\Lcont$ satisfying certain homogeneous initial conditions is invertible if and only if the underlying system of differential equations has a dichotomy.
%Moreover, in that case the operator is proved to be a direct sum of two
%infinitesimal generators of $C_0$-semigroups, one of which has support on the
%negative half-line and the other on the positive half-line. The effect of perturbations
%of the initial values on the dichotomy is also described.

%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Infinite-dimensional case}

%Most recent efforts in this area are spent in trying to deal with unbounded operators $\Acont(t)$.
In the case of bounded operators $\Acont(t)$ for $I=\Rplus$, the exponential dichotomy for solutions was characterized in the monographs \cite{MASS__LIN_DIF_EQ_AND_FUNC_SPACES} and \cite{DALKREINSTAB} in terms of the surjectivity of $\Lcont$ and the closedness and complementability of the subspace of those vectors in $\Xcont$ that are the initial data of bounded solutions of \eqref{eqs:homcont} on $\Rplus$.

%%%%%%%%%%%%%%%%%%%%%%%  Dalecki, Krein

%Consider the case where $\Xdiscr$ is a Banach space, $\Icont = \Rplus$ and $\Mdiscr = C_b(\Rplus,X)$.
%Let operators $\Acont(t)$ be bounded.
%In \cite{DALKREINSTAB} Dalecki and Krein show that the operator $\Lcont$ is invertible and $\setdef{x(0)}{ x(t) = S(t)x(0),\ t > 0 \hbox{ and } x\in\Mcont}$ is complementable in $\Xcont$ if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rplus$.
%
%%%%%%%%%%%%%%%%%%%%%%%%  Massera
% see thm 5.3

%Consider the case where $\Xdiscr$ is a Banach space, $\Icont = \Rplus$ and $\Mdiscr = C_b(\Rplus,X)$.
%Let operators $\Acont(t)$ be bounded.
%In \cite{MASS__LIN_DIF_EQ_AND_FUNC_SPACES} Massera and Sch\"{a}ffer show that the operator $\Lcont$ is invertible and $\setdef{x(0)}{ x(t) = S(t)x(0),\ t > 0 \hbox{ and } x\in\Mcont}$ is complementable in $\Xcont$ if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rplus$.

% precise statements from Krein and Massera

%Maizel, dich eq inv on full line

\subsubsection{D. Henry} %Daniel
%%%%%%%%%%%%%%%%%%%%%%% Henry

Consider the case where $\Xdiscr$ is a Banach space, $\Idiscr = \Zb$ and $\Mdiscr$ is  $\Lpdiscr{\infty}(\Zb,X).$
Let the sequence of operators $\Adiscr_k$ be bounded.
In \cite{HENRY__GEOM_TH_SMILIN_PARAB_EQ} Henry shows that the operator $\Ldiscr$ is invertible if and only if system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb.$

\subsubsection{V. Zhikov} %Vasiliy
%%%%%%%%%%%%%%%%%%%%%%%  Zhikov

Consider the case where $\Xcont$ is a separable Banach space, $\Icont = \Rplus$ and $\Mcont=C(\Rb,\Xcont)$ with standard $\sup$ norm.
Assume that also operator $\Lcont$ satisfy certain "right solvability" condition and the family $\Phi(t,s)$ has exponential growth.
In \cite{ZHIKOV__ADMISS_DICH_QUESTIONS} Zhikov shows that under this assumptions $\Lcont$ is invertible if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rplus$.

% about correctness

\subsubsection{V. Slyusarchuk} %Vasiliy
%%%%%%%%%%%%% Slyusarchuk

In \cite{SLYUS__EXP_DICH_SOL_DICR_SYSTEMS} Slyusarchuk considers the case where $\Idiscr = \Zb$ and $\Adiscr_k$ maps one Banach space $\Xdiscr_k$ to another $\Xdiscr_{k+1}.$ Operator $\Ldiscr$ acts on space $\Mdiscr$ of sequences $\seqz{x}{k}$ with bounded norm $\normban{x}_{\Mdiscr} = \sup_{k\in\Zb} \normban{x(k)}$ to itself. Slyusarchuk shows that analog of the system \eqref{eqs:homdiscr} has exponential dichotomy if and only if the operator $\Ldiscr$ has a continuous inverse.

\subsubsection{A. Baskakov et al.} %Andrey
%%%%%%%%%%%%%%%%%%%%%%  Baskakov

Consider the case where $\Xdiscr$ is a Banach space, $\Idiscr = \Zb$ and $\Mdiscr$ is either $\Lpdiscr{p}(\Zb,X),$ where $p\in[1,\infty],$ or $c_0(\Zb,X).$
Let the sequence $\Adiscr_k$ be bounded.
In \cite{BASK__INV_FREDHOLM_PROPS_DIF_OPER_00} Baskakov shows that the operator $\Ldiscr$ is invertible if and only if system \eqref{eqs:homdiscr} is dichotomic on both $\Zminus \setminus \{ 0 \}$ and $\Zplus$ with projectors $P^-$ and $P^+,$ and $(I-P^+)\Adiscr_0(I-P^-)$ is an isomorphism mapping $(I-P^-)\Xdiscr$ to $(I-P^+)\Xdiscr.$

Consider the case where $\Xdiscr$ is a Banach space, $\Idiscr = \Zb$ and $\Mdiscr$ is either $\Lpdiscr{p}(\Zb,X),$ where $p\in[1,\infty].$
Let $\Adiscr_n$ be a family of closed linear operators with domains $D(\Adiscr_k)$ dense in $\Xdiscr.$ Let $\Ldiscr$ be an operator from $D(\Ldiscr)\subset \Lpdiscr{p}(\Zb,\Xdiscr)$ to $\Lpdiscr{p}(\Zb,X).$ Assume that the family $\Phi_{t,s}$ has exponential growth.
In \cite{BASK__SPEC_ANAL_WEIGHT_SHIFT_OPER_01} Baskakov and Pastukhov show that the operator $\Ldiscr$ is invertible if and only if system \eqref{eqs:homdiscr} have exponential dichotomy on $\Zb$. In \cite{BASK__SPEC_ANAL_WEIGHT_SHIFT_OPER_01} the similar statement for continuous case is also proved.

%
%And similar for continuous case:
%The operators $\Acont(t) : D(\Acont(t)) \subset \Xcont \to \Xcont$ are assumed to be closed and generating a correct Cauchy problem on $\Rplus.$
%Then if $\Lcont$ maps $D(\Lcont)\subset \Lpcont{p}$ to $\Lpcont{p}$ with $p\in[1,\infty]$ then it is invertible if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rb$.

% Theorem 1.4, E=X, there is also a condition that Im Q(0) = E = X. That might be not interesting
%Consider the case where $\Icont = \Rb+.$  Baskakov in \cite{BASK__SPEC_ANAL_DEFF_OPER_UNBOUND_COEF}  studies different properties of operator $\Lcont$ including its invertibility and Fredholm properties for so-called homogeneous spaces. Examples of homogeneous spaces are $L^p(\Rplus,X),\ p\in[0,\infty]$ with standard norm, the space of bounded continuous functions $C_b(\Rplus,X)$ with $sup$ norm, the space $C_{0,b}(\Rplus,X) \subset C_b(\Rplus,X)$ of bounded continuous functions with $\lim_{t\to \infty} \normban{x(t)} \to 0,$ Stepanov spaces and $L^{p,q}$ spaces.

% Corollary 1.3
Consider the case where $\Xdiscr$ is a Banach space, $\Icont = \Rplus$ and $\Mdiscr$ is homogeneous space. For the definition of homogeneous spaces see \cite{MASS__LIN_DIF_EQ_AND_FUNC_SPACES, BASK__SPEC_ANAL_DEFF_OPER_UNBOUND_COEF_09}. The concept of homogeneous space generalizes $C_b,$ $C_0$ and $\Lpcont{p}.$
Let operators $\Acont(t) : D(\Acont(t)) \subset \Xcont \to \Xcont$ be closed. Assume that the family $\Phi_{t,s}$ has exponential growth.
%$\Phi(s,t)$ solve solve the abstract Cauchy problem \eqref{eqs:homcont}.
In \cite{BASK__SPEC_ANAL_DEFF_OPER_UNBOUND_COEF_09} Baskakov shows that the operator $\Lcont$ is invertible and $\setdef{x(0)}{ x(t) = S(t)x(0),\ t > 0 \hbox{ and } x\in\Mcont}$ is complementable in $\Xcont$ if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rplus$.
% Baskakov generalizes some results of N. Van Minh

The same is proved in \cite{DALKREINSTAB} for the case of bounded operator-valued coefficients on $C_b(\Rplus,\Xcont)$ and in \cite{MASS__LIN_DIF_EQ_AND_FUNC_SPACES} for the same operators on spaces of measurable functions (including $\Lpcont{p}(\Rplus,\Xcont),$ where $p \in [1,\infty]).$ The similar (if we are do not care about the precise statements) is done in \cite{NVM__EXP_STAB_EXP_EXPANS_EXP_DICH_HALFLINE_98, NVM__CHAR_DICH_EVOL_FAM_HALFLINE_01} for the spaces $C_{b,0}(\Rplus,\Xcont)$ and $\Lpcont{p}(\Rplus,\Xcont),$ where $p \in [1,\infty)$.

%%%%%%%%%%%%%%%%%%%%%%% N. Van Minh

%Consider the case where $\Xcont$ is a Banach space, $I = \Rplus,$ and $M$ is either $\Lpcont{p}(\Rplus,X),\ 1\leq p < \infty$ or $C_0(\Rplus,X).$
%Assume that $\Acont(t)$ is bounded and continuous.
%In \cite{NVM__EXP_STAB_EXP_EXPANS_EXP_DICH_HALFLINE_98} and
%\cite{NVM__CHAR_DICH_EVOL_FAM_HALFLINE_01} it is shown that system \eqref{eqs:homcont}
%has exponential dichotomy on $\Rplus$ if and only if the operator $\Lcont$ is surjective and the space $\dim \setdef{ u(0) }{ u \in \ker \Lcont  } $ is complemented in $\Xcont.$

% find what cite Nguen

\subsubsection{Yu. Latushkin et al.} %Yuri
%%%%%%%%%%%%%%%%%%%%%%% Latushkin

%Theorem 5.5.
Consider the case where $\Xcont$ is a Banach space, $I = \Rplus,$ and $M$ is either $\Lpcont{p}(\Rplus,X),$ where $1\leq p < \infty$ or $C_0(\Rplus,X).$  Let all $\Phi(s,t)$ be invertible operators and assume that the family $\Phi_{t,s}$ has exponential growth.
In \cite{LAT__FRED_PROP_EVOL_SEMIGROUPS_04} Latushkin shows that the following conditions are equivalent:
\begin{itemize}
\item the operator $\Lcont$ is Fredholm;
\item system \eqref{eqs:homcont} has an exponential dichotomy on $\Rplus$ with projection $P$ and $\dim \mathrm{Im} P < \infty;$
\item the operator $\Lcont$ is surjective and $\dim \setdef{ u(0) }{ u \in \ker \Lcont  } < \infty. $
\end{itemize}

Consider the case where $\Xcont$ is a Banach space, $I=\Rb$ and $\Mcont$ is either $\Lpcont{p}(\Rb,\Xcont),$ where $p\in[0,\infty)$ or $C_0(\Rb,\Xcont).$
Assume that $\Phi(s,t)$ solving the equation \eqref{eqs:homcont} in a mild sense. Assume that the family $\Phi_{t,s}$ has exponential growth.
In \cite{LAT__DICH_FRED_PROPS_EVOL_EQ_07} Latushkin shows that the operator $\Lcont$ is Fredholm if and only if there exist real numbers $a\leq b$ such that system \eqref{eqs:homcont} have exponential dichotomies on $(-\infty,a]$ and $[b,\infty)$ with projectors $P^+$ and $P^-$ and the node operator $N(a,b)=(I-P^+)\Phi(b,a)\vert_{\ker P^-} : \ker P^- \to \ker P^+$ is Fredholm. The same is proved in \cite{LAT__FRED_DIF_OPER_UNBOUND_COEF_05} with some additional conditions.

Consider the case where $X$ is a Hilbert space, $\Icont = \Rb$ and $\Mcont = L_2(\Rb,\Xcont).$ Let assume that the family $\Phi_{t,s}$ has exponential growth.
In \cite{LAT__DICH_TH_EVOL_BIFAM_08} Latushkin shows that the operator $\Lcont$ is Fredholm if and only if the not well-posed equation \eqref{eqs:homcont} has exponential dichotomies on both $\Rplus$ and $\Rminus$ and the ranges of the dichotomy projections form a Fredholm pair.

\subsubsection{B. Sasu et al.} %Bogdan
%%%%%%%%%%%%%%%%%%%%%%% Bogdan Sasu

%% study admissibility and connections to dichotomy and tricotomy in different functional spaces

Consider the case where $\Xdiscr$ is a Banach space, $\Icont = \Zplus.$
For a Banach space $B$ denote
$$X_{0,B} = \setdef{x_0}{ x_k = S_kx_0,\ k > 0 \hbox{ and } x\in B}.$$
In
\cite{SASU__DISCR_ADMISS_EXP_DICH_EVOL_FAM_03}, %Theorem 2.3
\cite{SASU__EXP_DICH_LPLQ_ADM_HALF_06}, %Theorem 2.1
\cite{SASU__UNIFORM_DICH_EXP_DICH_HALFLINE_06} % Theorem 4.1
%it is shown that
it is shown that if one considers the following conditions
\begin{enumerate}
\item \label{enumitem:expdich} system \eqref{eqs:inhomdiscr} has exponential dichotomy on $\Rplus;$

\item \label{enumitem:expgrowth} the family $\Phi_{s,t}$ has exponential growth;

\item \label{enumitem:lpadm}  the pair $(\Lpdiscr{p}(\Zplus,\Xdiscr),\Lpdiscr{q}(\Zplus,\Xdiscr)),$ where $p,q\in[1,\infty),$ is admissible for system \eqref{eqs:inhomdiscr} and the subspace $X_{0,\Lpdiscr{p}(\Zplus,\Xdiscr)}$ is closed and complemented in $X;$

\item \label{enumitem:c0adm} the pair $(c_0(\Zplus,\Xdiscr),c_0(\Zplus,\Xdiscr))$ is admissible for system \eqref{eqs:inhomdiscr} and the subspace $X_{0,c_0(\Zplus,\Xdiscr) }$ is closed and complemented in $X;$

\item \label{enumitem:linfadm} if the pair $(\Lpdiscr{\infty}(\Zplus,\Xdiscr),\Lpdiscr{p}(\Zplus,\Xdiscr)),$ where $p\in(1,\infty]$ is admissible for system \eqref{eqs:inhomdiscr} and the subspace $X_{0,\Lpdiscr{\infty}(\Zplus,\Xdiscr)}$ is closed and complemented in $X,$
\end{enumerate}
then
\begin{itemize}
\item \ref{enumitem:lpadm} implies \ref{enumitem:expdich},
\item \ref{enumitem:c0adm} implies \ref{enumitem:expdich},
\item \ref{enumitem:linfadm} implies \ref{enumitem:expdich},
\item \ref{enumitem:expgrowth} and \ref{enumitem:lpadm} for $p\geq q$ are equivalent to \ref{enumitem:expdich},
\item \ref{enumitem:expgrowth} and \ref{enumitem:c0adm} are equivalent to \ref{enumitem:expdich},
\item \ref{enumitem:expgrowth} and \ref{enumitem:linfadm} are equivalent to \ref{enumitem:expdich}.
\end{itemize}

%The same is proved for the continuous case.

%%

In \cite{SASU__EXP_DICH_FULL_LINE_ADMISS_FUNC_SP_06} the notion of translation invariant space is introduced. This notion generalizes $C_b,$ $C_0$ and $L_p$ spaces. In particular Orlicz spaces with certain additional restrictions are translation invariant.

Consider the case where $\Xcont$ is a Banach space, $\Icont = \Rb.$
Fix $p,q\in[1,\infty).$ Denote $X_0 = \setdef{x_0}{ x_k = S_kx_0,\ t > 0 \hbox{ and } x\in }.$
Assume that the family $\Phi_{s,t}$ has exponential growth. Let $B$ be a %\textit{good}
translation-invariant subspace containing $C(\Rb,X)$ and satisfying $B\setminus\Lpcont{1} \neq \emptyset.$ In  \cite{SASU__EXP_DICH_FULL_LINE_ADMISS_FUNC_SP_06} it is shown that under these assumptions if the pair $(C_b(\Rb,\Xcont),B(\Rb,\Xcont))$ is admissible for the system \eqref{eqs:inhomcont} then system \eqref{eqs:homcont}
has exponential dichotomy on $\Rb.$

In  \cite{SASU__EXP_DICH_FULL_LINE_ADMISS_FUNC_SP_06} it is also shown that the pair $(C_b(\Rb,\Xcont),L^p(\Rb,\Xcont))$ is admissible for the system \eqref{eqs:inhomcont} if and only if system \eqref{eqs:homcont} has exponential dichotomy on $\Rb.$
The similar holds when one replaces $\Lpcont{p}$ with Orlicz subspace with certain additional conditions.

\begin{deffnon}
We say that the pair $(U,V)$ of subspaces of $\Xcont^{\Icont}$ is uniformly admissible (see \cite{SASU__TRANS_INV_SPACES_ASYMPT_PROPS_VAR_EQ_11}) for the system \eqref{eqs:inhomdiscr} if there exist constant $C$ such that if for every inhomogeneity $f$ from $V$ there exist a solution $y$ of the system that belongs to $U$ and $\normban{y}_U \leq C\normban{f}_V.$ This is equivalent to saying (in some situations) that the operator $\Lcont$ is surjective and correct in the sense of Zhikov (see \cite{ZHIKOV__ADMISS_DICH_QUESTIONS}).
\end{deffnon}

Consider the case where $\Xdiscr$ is a Banach space, $\Icont = \Rplus.$
%Let $\Acont(t)$ be a family of densely defined closed operators.
Let $B$ be a %\textit{good}
translation-invariant space. Assume that the family $\Phi_{s,t}$ has exponential growth. In \cite{SASU__TRANS_INV_SPACES_ASYMPT_PROPS_VAR_EQ_11} it is shown that
\begin{itemize}
\item if the pair $(B(\Zb,\Xdiscr),B(\Zb,\Xdiscr))$ is uniformly admissible for system \eqref{eqs:inhomdiscr} then system \eqref{eqs:homdiscr} has exponential dichotomy on $\Rb;$
\item if $B$ is rearrangement invariant then the pair $(B,B)$ is uniformly admissible for system \eqref{eqs:inhomdiscr} if and only if system \eqref{eqs:homdiscr} has exponential dichotomy on $\Rb.$
\end{itemize}

%Let O. be an Orlicz space such that .(1) < Ѓ‡ and O.\L1(R,R) = ..

%%

Denote $\Delta(\Idiscr,\Xdiscr)=\setdef{ \seq{x_k}_{k\in\Idiscr} }{ \#\setdef{ k }{ x_k \neq 0 } < \infty }.$

Consider the case where $\Idiscr = \Zplus.$

\begin{deffnon}
Let $p, q \in[1,\infty].$ We say that the pair of spaces $(A,B)$ is uniformly $q$-admissible for system \eqref{eqs:inhomdiscr} if the following assertions hold:
\begin{itemize}
\item for every $f\in \Delta(\Zb,\Xdiscr)$ there is unique solution $y\in \Lpdiscr{p}$ of system \eqref{eqs:inhomdiscr} with inhomogeneity $f$.
\item there exist a constant $C>0$ such that $\normban{y}_{\Lpdiscr{p} } \leq C\normban{\Lpdiscr{q}}.$
\end{itemize}
\end{deffnon}

Let $p, q \in[1,\infty]$ be such that $(p,q)\neq (1,\infty)$. In \cite{SASU__INP_OUTPUT_COND_ASYMP_BEHAVIOR_LIN_SKEW_PROD_06} it is shown that the following assertions hold:
\begin{itemize}
\item if the pair $( \Lpdiscr{p}(\Zb,\Xdiscr),\Delta(\Zb,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr} then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb$;
\item if $p\geq q$ and the family $\Adiscr(t)$ is bounded, then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb$ if and only if the pair $( \Lpdiscr{p}(\Zb,\Xdiscr),\Delta(\Zb,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr}.
\end{itemize}

%%
Consider the case where $\Idiscr = \Zplus.$
Assume that the family $\Phi_{s,t}$ has exponential growth. Let $p, q \in[1,\infty]$ be such that $(p,q)\neq (1,\infty)$.
In \cite{SASU__DICH_BEHAVIOR_VAR_DIF_EQ_09} it is shown that the following assertions hold:
\begin{itemize}
\item if the pair $( \Lpdiscr{p}(\Zplus,\Xdiscr),\Delta(\Zplus,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr} and stable and unstable subspaces span entire $\Xdiscr$ then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zplus$;
\item if $p\geq q$ then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zplus$ if and only if the pair $( \Lpdiscr{p}(\Zplus,\Xdiscr),\Delta(\Zplus,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr}.
\end{itemize}

%%

Consider the case where $\Idiscr = \Zplus.$
Assume that the family $\Phi_{s,t}$ has exponential growth. Let $p, q \in[1,\infty]$ be such that $(p,q)\neq (1,\infty)$.
In \cite{SASU__DICH_BEHAVIOR_VAR_DIF_EQ_09} it is shown that the following assertions hold:
\begin{itemize}
\item if the pair $( \Lpdiscr{p}(\Zplus,\Xdiscr),\Delta(\Zplus,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr} and stable and unstable subspaces span entire $\Xdiscr$ then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zplus$;
\item if $p\geq q$ then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zplus$ if and only if the pair $( \Lpdiscr{p}(\Zplus,\Xdiscr),\Delta(\Zplus,\Xdiscr) )$ is uniformly $q$-admissible for the system \eqref{eqs:inhomdiscr}.
\end{itemize}

%%

Consider the case where $\Idiscr = \Zb.$
%Theorem 4.6
Let $A,B$ be two Orlicz spaces. In \cite{SASU__INP_OUT_CONTROL_SYS_DICH_VAR_DIF_EQ_11} it is also shown that if $(A,B)\neq (\Lpdiscr{\infty},\Lpdiscr{1})$ then the following assertions hold:
\begin{itemize}
\item if the pair $(A(\Zb,\Xdiscr),B(\Zb,\Xdiscr))$ is admissible for the system \eqref{eqs:inhomdiscr}, then system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb$;
\item if $B \subset A$ then the system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb$ if
and only if the pair $(A(\Zb,\Xdiscr),B(\Zb,\Xdiscr))$ is admissible for the system \eqref{eqs:inhomdiscr}.
\end{itemize}

%%

Consider the case where $\Idiscr = \Zb.$
%Theorem 4.7
Let $p, q \in [1,\infty].$ In \cite{SASU__INP_OUT_CONTROL_SYS_DICH_VAR_DIF_EQ_11} it is also shown that the following assertions hold:
\begin{itemize}
\item if the pair $(\Lpdiscr{q}(\Zb,\Xdiscr),\Lpdiscr{p}(\Zb,\Xdiscr))$ is admissible for system \eqref{eqs:inhomdiscr}, then the system \eqref{eqs:homdiscr} is
uniformly dichotomic;
\item if $(p,q)\neq (1,\infty)$ and the pair $(\Lpdiscr{q}(\Zb,\Xdiscr),\Lpdiscr{p}(\Zb,\Xdiscr))$ is admissible for  system \eqref{eqs:inhomdiscr}, then  system \eqref{eqs:homdiscr} is uniformly exponentially dichotomic;
\item if $(p,q)\neq (1,\infty)$ and $p \leq q$, then  system \eqref{eqs:homdiscr} is uniformly exponentially
dichotomic if and only if the pair $(\Lpdiscr{q}(\Zb,\Xdiscr),\Lpdiscr{p}(\Zb,\Xdiscr))$ is admissible for  system
\eqref{eqs:inhomdiscr}.
\end{itemize}

Consider the case where $\Idiscr = \Zb.$
%Theorem 4.8
Let $B$ be translation invariant. In \cite{SASU__INP_OUT_CONTROL_SYS_DICH_VAR_DIF_EQ_11} it is shown that then system \eqref{eqs:homdiscr} has exponential dichotomy on $\Zb$
and only if the pair $(B(\Zb,\Xdiscr),B(\Zb,\Xdiscr))$ is admissible for the system \eqref{eqs:inhomdiscr}.

%%%%%%%%%%%%%%%%%%%%%



%L R - strictly bigger than L1
%Q R - translation such that sup norm of chi([0,t]) = infty


\subsubsection{M. Bichegkuev} %Mairbek
%%%%%%%%%%%%%%%%%%%%%%% Bichegkuev

Let $\alpha = \seq{\alpha_k}_{k\in\Zplus}$ be a sequence of positive real numbers. Denote
$$
\normban{x}_{p,\alpha} = \enbrace{ \sum_{k=0}^{\infty} \enbrace{\frac{\normban{ x_k }}{\alpha_k } }^p }^{ \frac{1}{p} } ,\quad p\in[0,\infty);
$$

$$
\normban{x}_{\infty,\alpha} = \sup_{k\in\Zplus} \frac{\normban{ x_k }}{ \alpha_k };
$$

$$
\Lpdiscr{p}^{\alpha}(\Rplus,\Xdiscr)=\setdef{ \seq{x_k} }{ \normban{\seq{x_k}}_{p,\alpha} < \infty },\ p\in[0,\infty].
$$

Consider the case where $X$ is a Banach space, $\Idiscr = \Zplus$ and $\Mdiscr = \Lpdiscr{p}^{\alpha}(\Rplus,\Xdiscr),\ p\in[0,\infty].$
Assume that $A_k=B,\ k\in\Zplus,$ where $B$ is a bounded linear operator.
%
In \cite{BICHEG_COND_INVERT_DIF_OPER} Bichegkuev characterizes the invertibility of the operator $\Ldiscr$ in terms of growth rate of $\seq{\alpha_k},$ spectral properties of the operator $B$ and surjectivity of one of the spectral projections.

%%%%%%%%%%%%%%%%%%%%%%%

See more references in \cite{BASK__SPEC_ANAL_DEFF_OPER_UNBOUND_COEF_09, LAT__FRED_PROP_EVOL_SEMIGROUPS_04, LAT__DICH_FRED_PROPS_EVOL_EQ_07}.


% Latushkin book
% http://books.google.ru/books?id=4UH8K_vKktkC&pg=PA1&lpg=PA1&dq=Evolution+semigroups+in+dynamical+systems+and+differential+equations&source=bl&ots=gVvIg1tgVU&sig=Yv_Ky5A_r5Fk_anhiJYi0-ociDk&hl=ru&sa=X&ei=7Bo4T9nqNIvXsgbB_-W4DA&ved=0CEEQ6AEwAw#v=onepage&q=semigroup&f=false

%Results related to this property are widely used in different areas: for study of existence of transversal homoclinic orbits of perturbed differential systems (ZENG) (see  PALMER, ZENG), for study different robustness properties in both finite dimensional and infinite dimensional cases (PALMER, Barriera, Popescu, Latushkin),
%
%there is an important connection of the Dichotomy Theorem and the celebrated
%Atiyah-Patodi-Singer \Index=Spectral Flow" Theorem, see [3,35].
%(35] J. Robbin and D. Salamon, The spectral
%ow and the Maslov index, Bull. London Math. Soc. 27
%(1995), 1{33.)
%
%[3] M. F. Atiyah, V. K. Patodi and I. M. Singer, Spectral asymmetry and Riemannian geometry, Math.
%Proc. Cambridge Philos. Soc. 79 (1976), 79-99.

%From Barriera 2008
%To obtain a criterion for the existence of nonuniform exponential dichotomies one can also
%use a Fredholm alternative for the nonlinear perturbations. In particular, related work is due to
%Palmer [24] for ordinary differential equations, Lin [18] for functional differential equations,
%Blбzquez [7], Rodrigues and Silveira [30], Zeng [33] and Zhang [34] for parabolic evolution
%equations, and Chow and Leiva [9], Sacker and Sell [31] and Rodrigues and Ruas-Filho [29] for
%abstract evolution equations.



Василий Слюсарчук



==> sublinsh_backproof_full.tex <==
\subsection{Доказательство в обратную сторону}


\begin{deff} Последовательность $\mathcal{A}$ обладает $(C,\lambda)$ структурой с константами $C>1$ и $\lambda\in(0,1),$ если для любого целого $k$ существуют такие проекции $P_k, Q_k,$ что если $S_k=P_k\Rb^d$ и $U_k=Q_k\Rb^d,$ то выполняется следующее: 
\begin{IEEEeqnarray}{c}
\Rb^d=S_k \oplus  U_k; \\
A_kS_k \subset S_{k+1},\ A_kU_k \subset U_{k+1};  \label{clambdadef:subset}\\
|\Phi_{k,l}v|\leq C\lambda^{k-l}|v|,\ v\in S_l,\ k\geq l; \label{clambdadef:stable}\\
|\Phi_{k,l}v|\leq C\lambda^{l-k}|v|,\ v\in U_l,\ k\leq l; \label{clambdadef:unstable}\\
\normop{P_k},\normop{Q_k} \leq C. \label{clambdadef:projbound}
\end{IEEEeqnarray}
Здесь везде имеется в виду, что индексы пространств лежат в $[a,b].$
\end{deff}

\begin{rem}
Единственное отличие этого определения от определения гиперболичности в том, что в  \eqref{clambdadef:subset} стоят знаки включения, а не равенства.
\end{rem}

\begin{rem} \label{rem:clambdabound_omega}
Аналогично замечанию \ref{rem:hyperbound_omega}, для любого вещественного $\omega$ выполнение условий \eqref{clambdadef:stable} и \eqref{clambdadef:unstable} равносильно тому, что существует такое $\lambda_1 \in (0,1),$ что выполняются следующие оценки
\begin{IEEEeqnarray*}{c}
|\Phi_{k,l}v|\leq K\lambda_1^{k-l}(k+1)^{-\omega} (l+1)^{\omega}|v|,\ v\in S_l,\ k\geq l; \\
|\Phi_{k,l}v|\leq K\lambda_1^{l-k}(k+1)^{-\omega} (l+1)^{\omega}|v|,\ v\in U_l,\ k\leq l. 
\end{IEEEeqnarray*}
Здесь также имеется в виду, что индексы всех пространств лежат в $[a,b].$
\end{rem}


% Лемма 2.2.16 из \cite{PILSDS} + гёльдеровость распределений

%написать, как строим пространства.

\begin{statement} \label{st:huge_ss_conseq}
Пусть $f$ -- структурно устойчивый диффеоморфизм гладкого замкнутого многообразия $M.$ Тогда для каждой точки $p$ из $M$ существуют такие подпространства $S(p),U(p)\subset T_p M,$ что выполнено следующее:

\begin{itemize}
\item $S(p)\oplus U(p) = T_p M;$
\item $Df(p) S(p) \subset S(f(p)),\quad Df^{-1}(p) U(p)\subset U(f^{-1}(p));$
\item Существуют такие константы $C_1>0$ и $\lambda_1 \in (0,1),$ что
$$\vmod{Df^k(p) v}\leq C_1\lambda_1^k \vmod{v},\quad v\in S(p),\ k\geq 0,$$
$$\vmod{Df^{-k}(p) v}\leq C_1\lambda_1^k \vmod{v},\quad v\in S(p),\ k\geq 0;$$
\item Существует константа $N,$ такая, что если $P(p)$ и $Q(p)$ - дополнительные друг другу проекторы, соответствующие $S(p)$ и $U(p),$ то
$$ \normop{P(p)}, \normop{Q(p)} ,\leq N; $$
\item Существуют такие константы $C_2>0,\ \omega\in (0,1),$  что для любого натурального $T$ существует такое число $\alpha > 0,$ что если $z,p\in M,\ q=f^T(p),\ y=f^{-T}(z)$ и $\dist(z,q)<\alpha,$ то существует такой линейный изоморфизм $\Pi(p,x):T_z M \to T_z M,$ что
$$ \normop{\Pi - I}\leq C_2\dist(z,q)^\omega,\ \Pi(p,z)(D(exp_z^{-1}(q) Df^{-T}(p) S(p)) \subset S(z), $$
и такой линейный изоморфизм $\Theta(p,z):T_p M \to T_p M,$ что
$$ \normop{\Theta - I}\leq C_2\dist(z,q)^\omega,\ \Theta(p,z)(D(exp_p^{-1}(y) Df^{-T}(z) U(z)) \subset U(p). $$

\end{itemize}
\end{statement}


\begin{lemmaa} \label{lemma:shfT_impl_shf}
Пусть $f$ -- $C^1$ гладкий диффеоморфизм $M$ и $T$ -- натуральное число. Если $f^T\in LSlSP(\gamma),$ то также $f\in LSlSP(\gamma).$  %см lemma 1.1.3 у в shadowbook
\end{lemmaa}
\begin{proof}
Аналогично доказательству леммы 1.1.3 в \cite{PILSDS}.
\end{proof}

% Теорема 2.2.7 из \cite{PILSDS}.

\begin{theorem}
Пусть $f$ -- структурно устойчивый $C^{1+\delta} $диффеоморфизм гладкого замкнутого многообразия $M.$ Тогда для любого $\gamma \geq 0$ выполнено, что $f\in LSlSP(\gamma).$
\end{theorem}

\begin{proof}
Выберем такое $T,$ чтобы $$\mu = C\lambda_1^T < 1.$$
По лемме \ref{lemma:shfT_impl_shf} для того, чтобы доказать, что $f\in LSlSP(\gamma),$ достаточно доказать, что $f'=f^T\in LSlSP(\gamma).$
Воспользуемся утверждением \ref{st:huge_ss_conseq} при $C=1,\ \lambda_1 = \mu$ и $T=1.$

Возьмём такое $\nu_0 \in (0,1),$ чтобы $\lambda = (1+\nu_0)^2\mu < 1.$ 
%Для этого $\lambda$ и числа $N$ из утверждения \ref{st:huge_ss_conseq} выберем такое $\kappa>0,$ что $\kappa N_1 < 1.$ 
Обозначим
$$K=\max(N,\max_{p\in M}\normop{Df(p)},\max_{p\in M}\normop{Df^{-1}(p)}).$$
Найдём такое число $\nu \in (0,\nu_0),$ что 
$$ 2K(2K+1)\nu < \kappa/2. $$

Пусть $c$ -- такой радиус, что для всех $p\in M$ отображения $\exp_p$ являются диффеоморфизмами шара $E_{2c}(p)\subset T_p M$ на его образ. Берём такое число $d' < c,$ что для всех точек $x,y \in M$ при $\dist(x,y) \leq d'$ и $y'=\exp_x^{-1}(y)$ выполнены неравенства
%(можно просто уменьшить $c$ и не вводить новую букву)
$$
\vmod{D\exp_x^{-1}(y) v} \leq (1+\nu) \dist(x,y)^{\omega_2},
$$
$$
\vmod{D\exp_x (y') v} \leq (1+\nu) \dist(x,y')^{\omega_2}.
$$
% так как Dexp_x(x) = Id и многообразие C^\infty

Уменьшим $d'$ так, чтобы оно работало в качестве $\alpha$ из утверждения $\ref{st:huge_ss_conseq}.$

Пусть $x_k$ это $\sigma$-$d$-псевдотраектория при $d\leq d'.$ 

Определим отображения $f_k:T_{x_k} \to T_{x_{k+1}}$ формулой
$$ f_k = \exp_z^{-1} \circ f \circ \exp_p. $$
Тогда отображения $f_k$ определены на $E_{d'}(x_k).$ Очевидно, что
$$|f_k(0)|\leq d(|k|+1)^{-\gamma}.$$ % тк у нас pst

Введём следующие обозначения:
$$ p=x_k,\ \hat{p}=f(x_k)=f(p),\ z=x_{k+1}, $$
$$\check{z} = f^{-1}(x_{k+1})=f^{-1}(z),\ \check{z}' = 
\exp_p^{-1}(\check{z}) = \exp_{x_k}^{-1} (f^{-1} (x_{k+1})). $$
Обозначим $J_k=Df_k(0).$ Тогда
$$ J_k = D\exp_z^{-1}(\hat{p}) Df(p) = D\exp_{x_{k+1}}^{-1} (f(x_k)) Df(x_k). $$

Обозначим $F_k = Df(\check{z})D\exp_p (\check{z}') = Df(f^{-1}(x_{k+1}))D\exp_p (\exp_{x_k}^{-1} (f^{-1} (x_{k+1}))).$
Положим 
$$ A_k^s = \Pi (p,z)J_kP(p),\ A_k^u = F_k\Theta^{-1} (p,z) Q(p),\ A_k = A_k^s + A_k^u. $$

Хотим доказать, что последовательность $\{A_k\}$ обладает $(C,\lambda)$ структурой. Тогда можно воспользоваться теоремой на странице 10 статьи \cite{PILGNH}.

Представим $f_k$ в виде
$$ f_k(v) = J_k v + \chi(v),$$
где $\chi(0)=f_k(0),\ D\chi(0)=0.$ Так как дифференциалы $f$ и $\exp_p$ равномерно ограничены, можно уменьшить $d'$ так, чтобы выполнялось
$$ \vmod{\chi(v) - \chi(v')} \leq \frac{\kappa}{2} \vmod{v-v'},\ v,v' \in E_{d'}(p) \cap (S(p)\oplus U(p)) . $$


Пусть $v^s \in S(p).$ По построению пространств (на самом деле по леммам), $v_1=Df(p)v^s \in S(\hat{p})$ и $\vmod{v_1^s}\leq \mu\vmod{v^s}.$

\end{proof}


==> sublinsh_intro.tex <==


The theory of shadowing of approximate trajectories (pseudotrajectories)
of dynamical systems is now a well developed part of the global theory of
dynamical systems (see, for example, the monographs \cite{PILSDS, PALSDS}). In particular the connections between shadowing and structural stability are interesting.

It is well known that a structurally stable system has shadowing property and this property is Lipschitz (see \cite{PILSDS}). Recently it was shown that Lipschitz shadowing implies structural stability (see \cite{PILTIKLSISS}). Also structural stability follows from H\"{o}lder shadowing property under some additional assumptions (see \cite{TIKHHOL}). Moreover it is known that structurally stable system has two-sided limit shadowing property but even the $C^1$-interior of the set of diffeomorphisms having two-sided shadowing property (without prescribing the speed of convergence to zero of estimates on each step) not coincide with the set of structurally stable diffeomorphisms (see \cite{PILLMSP}).

We show that Lipschitz two-sided limit shadowing property is equivalent to structural stability. 

==> sublinsh_methods.tex <==
\subsection{Методы}

Наши доказательства используют два известных результата, принадлежащие Р. Мане и В. А. Плиссу. Сформулируем их.


Рассмотрим семейство линейных изоморфизмов
\begin{equation*}
\Ac=\{A_k:{\Rb}^d\to{\Rb}^d,\;k\in{\Zb}\}
\end{equation*}
и предположим, что существует такая константа $N>0$, что
$\|A_k\|,\|A^{-1}_k\|\leq N.$

Для установления структурной устойчивости мы показываем, что дифференциалы диффеоморфизмов, обладающих соответствующим свойством отслеживания, удовлетворяют условию теоремы Плисса (или условию её обобщения на случай убывающих последовательностей в случае убывающего отслеживания) и потом применяем теорему Мане. 

